Extracting Social Determinants of Health from Pediatric Patient Notes Using Large Language Models: Novel Corpus and Methods

Social determinants of health (SDoH) play a critical role in shaping health outcomes, particularly in pediatric populations where interventions can have long-term implications. SDoH are frequently studied in the Electronic Health Record (EHR), which provides a rich repository for diverse patient data. In this work, we present a novel annotated corpus, the Pediatric Social History Annotation Corpus (PedSHAC), and evaluate the automatic extraction of detailed SDoH representations using fine-tuned and in-context learning methods with Large Language Models (LLMs). PedSHAC comprises annotated social history sections from 1,260 clinical notes obtained from pediatric patients within the University of Washington (UW) hospital system. Employing an event-based annotation scheme, PedSHAC captures ten distinct health determinants to encompass living and economic stability, prior trauma, education access, substance use history, and mental health with an overall annotator agreement of 81.9 F1. Our proposed fine-tuning LLM-based extractors achieve high performance at 78.4 F1 for event arguments. In-context learning approaches with GPT-4 demonstrate promise for reliable SDoH extraction with limited annotated examples, with extraction performance at 82.3 F1 for event triggers.

==> tables/annotator_agreement.tex <==




\scriptsize
\begin{tabular}{lrrr}\toprule
\textbf{Event Type} &\textbf{Argument type} &\textbf{F1} \\\midrule
Adoption &Trigger &1.000 \\
\multirow{2}{*}{Education access} &Trigger &0.800 \\
&Status &0.800 \\
\multirow{4}{*}{Living arrangement} &Trigger &0.905 \\
&Status &0.885 \\
&Type &0.884 \\
&Residence &0.381 \\
\multirow{2}{*}{Employment } &Trigger &0.811 \\
&Status &0.778 \\
\multirow{2}{*}{Food insecurity} &Trigger &0.400 \\
&Status &0.400 \\
\multirow{3}{*}{Trauma} &Trigger &0.889 \\
&Status &0.889 \\
&Type &0.846 \\
\multirow{3}{*}{Mental Health} &Trigger &0.667 \\
&Status &0.533 \\
&Experiencer &0.667 \\
\multirow{3}{*}{Substance use - alcohol/drug/tobacco} &Trigger &0.864 \\
&Status &0.857 \\
&Experiencer &0.732 \\
\multirow{3}{*}{Overall} &Trigger &0.851 \\
&Labeled arguments &0.800 \\
&All &0.819 \\
\bottomrule
\end{tabular}

==> tables/performance.tex <==





\newgeometry{left=2cm,right=2cm,top=2cm,bottom=2cm}
\begin{sidewaystable*}
\centering
\small
\setlength{\tabcolsep}{3pt}
%\begin{tabular}{ccccccccccccccccccccccccc}
\begin{tabular}{ccccccccccccccccccccccccc}
\hline
\multirow{2}{*}{\textbf{Event type}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Triggers / \\ Arguments\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# gold \\ labels\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}IAA\\ F1\end{tabular}}} & \multicolumn{9}{c}{\textbf{Fine-tuning approaches}} & \multicolumn{12}{c}{\textbf{GPT4}} \\ \cline{5-25} 
 &  &  &  & \multicolumn{3}{c}{\textbf{mSpERT}} & \multicolumn{3}{c}{\textbf{T5-Event}} & \multicolumn{3}{c}{\textbf{T5-Pipeline}} & \multicolumn{3}{c}{\textbf{GPT-Event}} & \multicolumn{3}{c}{\textbf{GPT-Pipeline}} & \multicolumn{3}{c}{\textbf{+ guideline}} & \multicolumn{3}{c}{\textbf{+ guideline + 3shot}} \\ \cline{5-25} 
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \hline
Adoption & Trigger & 9 & \multicolumn{1}{c|}{100.0} & 80.0 & 88.9 & \multicolumn{1}{c|}{84.2} & 87.5 & 77.8 & \multicolumn{1}{c|}{82.4} & 80.0 & 88.9 & \multicolumn{1}{c|}{\textbf{84.2}} & 40.9 & 100.0 & \multicolumn{1}{c|}{58.1} & 50.0 & 100.0 & \multicolumn{1}{c|}{66.7} & 50.0 & 100.0 & \multicolumn{1}{c|}{66.7} & 37.5 & 100.0 & 54.5 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Education\\ access\end{tabular}} & Trigger & 74 & \multicolumn{1}{c|}{80.0} & 82.1 & 74.3 & \multicolumn{1}{c|}{78.0} & 87.3 & 74.3 & \multicolumn{1}{c|}{80.3} & 90.6 & 78.4 & \multicolumn{1}{c|}{84.1} & 64.3 & 85.1 & \multicolumn{1}{c|}{73.3} & 77.5 & 74.3 & \multicolumn{1}{c|}{75.9} & 86.1 & 83.8 & \multicolumn{1}{c|}{84.9} & 79.3 & 93.2 & \textbf{85.7} \\
 & Status & 74 & \multicolumn{1}{c|}{80.0} & 82.1 & 74.3 & \multicolumn{1}{c|}{78.0} & 87.3 & 74.3 & \multicolumn{1}{c|}{80.3} & 90.6 & 78.4 & \multicolumn{1}{c|}{\textbf{84.1}} & 73.8 & 79.7 & \multicolumn{1}{c|}{76.6} & 69.6 & 43.2 & \multicolumn{1}{c|}{53.3} & 87.3 & 83.8 & \multicolumn{1}{c|}{85.5} & 78.2 & 91.9 & 84.5 \\ \hline
\multirow{2}{*}{Employment} & Trigger & 117 & \multicolumn{1}{c|}{81.1} & 83.3 & 68.4 & \multicolumn{1}{c|}{75.1} & 82.5 & 80.3 & \multicolumn{1}{c|}{81.4} & 83.6 & 78.6 & \multicolumn{1}{c|}{81.1} & 76.9 & 76.9 & \multicolumn{1}{c|}{76.9} & 75.0 & 71.8 & \multicolumn{1}{c|}{73.4} & 88.2 & 82.9 & \multicolumn{1}{c|}{85.5} & 83.6 & 95.7 & \textbf{89.2} \\
 & Status & 117 & \multicolumn{1}{c|}{77.8} & 79.2 & 65.0 & \multicolumn{1}{c|}{71.4} & 78.1 & 76.1 & \multicolumn{1}{c|}{77.1} & 80.2 & 69.2 & \multicolumn{1}{c|}{74.3} & 33.7 & 29.9 & \multicolumn{1}{c|}{31.7} & 67.6 & 60.7 & \multicolumn{1}{c|}{64.0} & 81.7 & 72.6 & \multicolumn{1}{c|}{76.9} & 76.3 & 85.5 & \textbf{80.6} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Food \\ insecurity\end{tabular}} & Trigger & 8 & \multicolumn{1}{c|}{40.0} & 100.0 & 87.5 & \multicolumn{1}{c|}{93.3} & 87.5 & 87.5 & \multicolumn{1}{c|}{87.5} & 100.0 & 87.5 & \multicolumn{1}{c|}{\textbf{93.3}} & 50.0 & 62.5 & \multicolumn{1}{c|}{55.6} & 0.0 & 0.0 & \multicolumn{1}{c|}{0.0} & 58.3 & 87.5 & \multicolumn{1}{c|}{70.0} & 72.7 & 100.0 & 84.2 \\
 & Status & 8 & \multicolumn{1}{c|}{40.0} & 100.0 & 87.5 & \multicolumn{1}{c|}{93.3} & 87.5 & 87.5 & \multicolumn{1}{c|}{87.5} & 100.0 & 87.5 & \multicolumn{1}{c|}{\textbf{93.3}} & 58.3 & 87.5 & \multicolumn{1}{c|}{70.0} & 0.0 & 0.0 & \multicolumn{1}{c|}{0.0} & 58.3 & 87.5 & \multicolumn{1}{c|}{70.0} & 87.5 & 87.5 & 87.5 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Living \\ arrangement\end{tabular}} & Trigger & 195 & \multicolumn{1}{c|}{90.4} & 90.2 & 80.0 & \multicolumn{1}{c|}{84.8} & 89.9 & 86.7 & \multicolumn{1}{c|}{\textbf{88.3}} & 86.8 & 84.1 & \multicolumn{1}{c|}{85.4} & 77.9 & 83.1 & \multicolumn{1}{c|}{80.4} & 84.0 & 77.9 & \multicolumn{1}{c|}{80.9} & 89.0 & 79.0 & \multicolumn{1}{c|}{83.7} & 86.0 & 82.1 & 84.0 \\
 & Status & 195 & \multicolumn{1}{c|}{88.5} & 87.9 & 77.9 & \multicolumn{1}{c|}{82.6} & 86.2 & 83.1 & \multicolumn{1}{c|}{\textbf{84.6}} & 87.0 & 82.1 & \multicolumn{1}{c|}{84.4} & 66.1 & 64.1 & \multicolumn{1}{c|}{65.1} & 81.7 & 75.4 & \multicolumn{1}{c|}{78.4} & 86.1 & 76.4 & \multicolumn{1}{c|}{81.0} & 80.5 & 76.4 & 78.4 \\
 & Type & 160 & \multicolumn{1}{c|}{88.4} & 73.4 & 79.4 & \multicolumn{1}{c|}{76.3} & 88.3 & 85.0 & \multicolumn{1}{c|}{86.6} & 91.9 & 85.6 & \multicolumn{1}{c|}{\textbf{88.7}} & 71.2 & 78.8 & \multicolumn{1}{c|}{74.8} & 73.4 & 77.5 & \multicolumn{1}{c|}{75.4} & 80.0 & 82.5 & \multicolumn{1}{c|}{81.2} & 76.5 & 79.4 & 77.9 \\
 & Residence & 38 & \multicolumn{1}{c|}{38.1} & 11.6 & 52.6 & \multicolumn{1}{c|}{19.0} & 77.4 & 63.2 & \multicolumn{1}{c|}{\textbf{69.6}} & 63.9 & 60.5 & \multicolumn{1}{c|}{62.2} & 20.5 & 81.6 & \multicolumn{1}{c|}{32.8} & 16.6 & 76.3 & \multicolumn{1}{c|}{27.2} & 17.2 & 76.3 & \multicolumn{1}{c|}{28.0} & 17.4 & 78.9 & 28.6 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mental \\ Health\end{tabular}} & Trigger & 15 & \multicolumn{1}{c|}{66.7} & 66.7 & 26.7 & \multicolumn{1}{c|}{38.1} & 44.4 & 26.7 & \multicolumn{1}{c|}{33.3} & 50.0 & 28.6 & \multicolumn{1}{c|}{36.4} & 19.5 & 53.3 & \multicolumn{1}{c|}{28.6} & 53.8 & 50.0 & \multicolumn{1}{c|}{51.9} & 50.0 & 57.1 & \multicolumn{1}{c|}{53.3} & 47.1 & 57.1 & \textbf{51.6} \\
 & Status & 15 & \multicolumn{1}{c|}{53.3} & 50.0 & 20.0 & \multicolumn{1}{c|}{28.6} & 44.4 & 26.7 & \multicolumn{1}{c|}{33.3} & 50.0 & 26.7 & \multicolumn{1}{c|}{34.8} & 15.4 & 26.7 & \multicolumn{1}{c|}{19.5} & 38.5 & 33.3 & \multicolumn{1}{c|}{35.7} & 37.5 & 40.0 & \multicolumn{1}{c|}{38.7} & 41.2 & 46.7 & \textbf{43.8} \\
 & Experiencer & 15 & \multicolumn{1}{c|}{66.7} & 16.7 & 6.7 & \multicolumn{1}{c|}{9.5} & 33.3 & 20.0 & \multicolumn{1}{c|}{25.0} & 25.0 & 13.3 & \multicolumn{1}{c|}{17.4} & 15.4 & 26.7 & \multicolumn{1}{c|}{19.5} & 38.5 & 33.3 & \multicolumn{1}{c|}{35.7} & 40.0 & 40.0 & \multicolumn{1}{c|}{40.0} & 41.2 & 46.7 & \textbf{43.8} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Substance use\\  - alcohol / \\ drug / tobacco\end{tabular}} & Trigger & 78 & \multicolumn{1}{c|}{86.4} & 92.5 & 79.5 & \multicolumn{1}{c|}{\textbf{85.5}} & 84.2 & 82.1 & \multicolumn{1}{c|}{83.1} & 89.4 & 75.6 & \multicolumn{1}{c|}{81.9} & 65.6 & 78.2 & \multicolumn{1}{c|}{71.3} & 76.8 & 55.1 & \multicolumn{1}{c|}{64.2} & 78.3 & 69.2 & \multicolumn{1}{c|}{73.5} & 71.7 & 91.0 & 80.2 \\
 & Status & 78 & \multicolumn{1}{c|}{85.7} & 88.1 & 75.6 & \multicolumn{1}{c|}{81.4} & 80.0 & 76.9 & \multicolumn{1}{c|}{78.4} & 89.4 & 75.6 & \multicolumn{1}{c|}{\textbf{81.9}} & 59.5 & 56.4 & \multicolumn{1}{c|}{57.9} & 76.4 & 53.8 & \multicolumn{1}{c|}{63.2} & 76.6 & 62.8 & \multicolumn{1}{c|}{69.0} & 68.7 & 87.2 & 76.8 \\
 & Experiencer & 78 & \multicolumn{1}{c|}{73.2} & 80.6 & 69.2 & \multicolumn{1}{c|}{74.5} & 81.6 & 79.5 & \multicolumn{1}{c|}{80.5} & 87.9 & 74.4 & \multicolumn{1}{c|}{\textbf{80.6}} & 59.2 & 37.2 & \multicolumn{1}{c|}{45.7} & 76.4 & 53.8 & \multicolumn{1}{c|}{63.2} & 76.8 & 67.9 & \multicolumn{1}{c|}{72.1} & 72.2 & 89.7 & 80.0 \\ \hline
\multirow{3}{*}{Trauma} & Trigger & 33 & \multicolumn{1}{c|}{88.9} & 72.0 & 54.5 & \multicolumn{1}{c|}{62.1} & 52.8 & 57.6 & \multicolumn{1}{r|}{55.1} & 59.3 & 48.5 & \multicolumn{1}{c|}{53.3} & 52.9 & 54.5 & \multicolumn{1}{c|}{53.7} & 50.0 & 3.0 & \multicolumn{1}{c|}{5.7} & 92.9 & 39.4 & \multicolumn{1}{c|}{55.3} & 83.3 & 60.6 & \textbf{70.2} \\
 & Status & 33 & \multicolumn{1}{c|}{88.9} & 60.0 & 45.5 & \multicolumn{1}{c|}{51.7} & 52.8 & 57.6 & \multicolumn{1}{c|}{55.1} & 61.5 & 48.5 & \multicolumn{1}{c|}{54.2} & 46.7 & 42.4 & \multicolumn{1}{c|}{44.4} & 50.0 & 3.0 & \multicolumn{1}{c|}{5.7} & 92.9 & 39.4 & \multicolumn{1}{c|}{55.3} & 75.0 & 54.5 & \textbf{63.2} \\
 & Type & 33 & \multicolumn{1}{c|}{84.6} & 64.0 & 48.5 & \multicolumn{1}{c|}{55.2} & 50.0 & 54.5 & \multicolumn{1}{c|}{52.2} & 61.5 & 48.5 & \multicolumn{1}{c|}{54.2} & 50.0 & 39.4 & \multicolumn{1}{c|}{44.1} & 50.0 & 3.0 & \multicolumn{1}{c|}{5.7} & 92.9 & 39.4 & \multicolumn{1}{c|}{55.3} & 79.2 & 57.6 & \textbf{66.7} \\ \hline
\multirow{3}{*}{\textbf{Overall}} & \textbf{--} & 1373 & \multicolumn{1}{c|}{81.9} & 73.0 & 71.0 & \multicolumn{1}{c|}{72.0} & 81.3 & 77.1 & \multicolumn{1}{c|}{79.1} & 84.2 & 75.0 & \multicolumn{1}{c|}{\textbf{79.3}} & 57.9 & 66.1 & \multicolumn{1}{c|}{61.7} & 66.6 & 62.0 & \multicolumn{1}{c|}{64.2} & 73.6 & 73.5 & \multicolumn{1}{c|}{73.5} & 70.0 & 82.1 & 75.6 \\
 & \textbf{Trigger} & 529 & \multicolumn{1}{c|}{85.1} & 86.5 & 73.7 & \multicolumn{1}{c|}{79.6} & 83.5 & 79.2 & \multicolumn{1}{c|}{81.3} & 84.8 & 77.3 & \multicolumn{1}{c|}{\textbf{80.9}} & 66.8 & 78.6 & \multicolumn{1}{c|}{72.2} & 76.8 & 66.5 & \multicolumn{1}{c|}{71.3} & 83.5 & 76.5 & \multicolumn{1}{c|}{79.8} & 78.5 & 86.6 & 82.3 \\
 & \textbf{Arguments} & 844 & \multicolumn{1}{c|}{80.0} & 66.1 & 69.3 & \multicolumn{1}{c|}{67.7} & 80.0 & 75.7 & \multicolumn{1}{c|}{77.8} & 83.8 & 73.6 & \multicolumn{1}{c|}{\textbf{78.4}} & 52.0 & 58.2 & \multicolumn{1}{c|}{54.9} & 60.9 & 59.1 & \multicolumn{1}{c|}{60.0} & 68.2 & 71.6 & \multicolumn{1}{c|}{69.8} & 65.2 & 79.4 & 71.6 \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hallucination \\ rate\end{tabular}}} & \textbf{Tigger} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{NA} & \multicolumn{3}{c|}{3.9} & \multicolumn{3}{c|}{3.9} & \multicolumn{3}{l|}{} & \multicolumn{3}{c|}{5.9} & \multicolumn{3}{c|}{5.4} & \multicolumn{3}{c}{4.1} \\
 & \textbf{Arguments} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{NA} & \multicolumn{3}{l|}{} & \multicolumn{3}{l|}{} & \multicolumn{3}{l|}{} & \multicolumn{3}{l|}{} & \multicolumn{3}{l|}{} & \multicolumn{3}{l}{} \\ \hline
\end{tabular}
\caption{Model performance (\%) on the test set. Hallucination rate stands for the percentage of invalid answers from generative models, including triggers that cannot be mapped to the original social history section and the arguments with undefined subtypes. IAA F1 (\%) stands for the last round of double annotation, which overlaps with the test set but is not the same as the test set. The best model IE F1 per row is highlighted in \textbf{bold}, with significantly better performance than all other models labeled by * (\textcolor{red}{to add the significance testing and complete the hallucination rate.})}
\label{tab:performance}
\end{sidewaystable*}
\restoregeometry





%\begin{tabular}{cccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{\textbf{Event type}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Triggers / \\ Arguments\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# gold \\ labels\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}IAA\\ F1\end{tabular}}} & \multicolumn{9}{c|}{\textbf{Fine-tuning approaches}} & \multicolumn{12}{c}{\textbf{In-context learning approaches with GPT4}} \\ \cline{5-25} 
%  &  &  &  & \multicolumn{3}{c|}{\textbf{mSpERT}} & \multicolumn{3}{c|}{\textbf{T5 text2event}} & \multicolumn{3}{c|}{\textbf{T5 multi-step QA}} & \multicolumn{3}{c|}{\textbf{Text2event}} & \multicolumn{3}{c|}{\textbf{Multi-step QA}} & \multicolumn{3}{c|}{\textbf{+ guideline}} & \multicolumn{3}{c}{\textbf{+ few-shot}} \\ \cline{5-25} 
%  &  &  &  & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \hline
 
% Adoption & Trigger & 9 & 100.0 & 80.0 & 88.9 & 84.2 & 87.5 & 77.8 & 82.4 & 88.9 & 88.9 & \textbf{88.9} & 40.9 & 100.0 & 58.1 & 50.0 & 100.0 & 66.7 & 37.5 & 100.0 & 54.5 & 37.5 & 100.0 & 54.5 \\ \hline %\cline{1-2}
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Education \\ access\end{tabular}} & Trigger & 74 & 80.0 & 82.1 & 74.3 & 78.0 & 87.3 & 74.3 & 80.3 & 95.1 & 78.4 & \textbf{85.9} & 64.3 & 85.1 & 73.3 & 84.9 & 83.8 & 84.4 & 78.8 & 74.5 & 76.6 & 79.3 & 93.2 & 85.7 \\
%  & Status & 74 & 80.0 & 82.1 & 74.3 & 78.0 & 87.3 & 74.3 & 80.3 & 90.6 & 78.4 & \textbf{84.1} & 73.8 & 79.7 & 76.6 & 72.7 & 32.4 & 44.9 & 86.1 & 83.8 & 84.9 & 77.0 & 90.5 & 83.2 \\ \hline %\cline{1-2}
 
% \multirow{2}{*}{Employment} & Trigger & 117 & 81.1 & 83.3 & 68.4 & 75.1 & 82.5 & 80.3 & 81.4 & 81.5 & 75.2 & 78.2 & 76.9 & 76.9 & 76.9 & 86.5 & 82.1 & 84.2 & 75.9 & 75.9 & 75.9 & 84.1 & 94.9 & \textbf{89.2} \\
%  & Status & 117 & 77.8 & 79.2 & 65.0 & 71.4 & 78.1 & 76.1 & 77.1 & 80.2 & 69.2 & 74.3 & 33.7 & 29.9 & 31.7 & 69.4 & 64.1 & 66.7 & 80.0 & 71.8 & 75.7 & 76.9 & 85.5 & \textbf{81.0} \\ \hline %\cline{1-2}
 
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Food \\ insecurity\end{tabular}} & Trigger & 8 & 40.0 & 100.0 & 87.5 & 93.3 & 87.5 & 87.5 & 87.5 & 100.0 & 87.5 & \textbf{93.3} & 50.0 & 62.5 & 55.6 & 58.3 & 87.5 & 70.0 & 50.0 & 14.3 & 22.2 & 72.7 & 100.0 & 84.2 \\
%  & Status & 8 & 40.0 & 100.0 & 87.5 & 93.3 & 87.5 & 87.5 & 87.5 & 100.0 & 87.5 & \textbf{93.3} & 58.3 & 87.5 & 70.0 & 0.0 & 0.0 & 0.0 & 63.6 & 87.5 & 73.7 & 87.5 & 87.5 & 87.5 \\ \hline %\cline{1-2}
 
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Living \\ arrangement\end{tabular}} & Trigger & 195 & 90.4 & 90.2 & 80.0 & 84.8 & 89.9 & 86.7 & \textbf{88.3} & 92.1 & 83.6 & 87.6 & 77.9 & 83.1 & 80.4 & 88.4 & 78.5 & 83.2 & 82.0 & 73.2 & 77.3 & 84.7 & 82.1 & 83.3 \\
%  & Status & 195 & 88.5 & 87.9 & 77.9 & 82.6 & 86.2 & 83.1 & \textbf{84.6} & 87.0 & 82.1 & 84.4 & 66.1 & 64.1 & 65.1 & 78.9 & 53.8 & 64.0 & 85.5 & 75.4 & 80.1 & 79.3 & 76.4 & 77.8 \\
%  & Type & 160 & 88.4 & 73.4 & 79.4 & 76.3 & 88.3 & 85.0 & 86.6 & 91.9 & 85.6 & \textbf{88.7} & 71.2 & 78.8 & 74.8 & 70.7 & 54.4 & 61.5 & 79.3 & 81.3 & 80.2 & 74.6 & 78.8 & 76.6 \\
%  & Residence & 38 & 38.1 & 11.6 & 52.6 & 19.0 & 77.4 & 63.2 & \textbf{69.6} & 63.9 & 60.5 & 62.2 & 20.5 & 81.6 & 32.8 & 14.1 & 47.4 & 21.7 & 17.2 & 76.3 & 28.0 & 17.2 & 78.9 & 28.3 \\ \hline % \cline{1-2}
 
% \multirow{3}{*}{Mental Health} & Trigger & 15 & 66.7 & 66.7 & 26.7 & 38.1 & 44.4 & 26.7 & 33.3 & 80.0 & 28.6 & 42.1 & 19.5 & 53.3 & 28.6 & 47.1 & 57.1 & 51.6 & 60.0 & 42.9 & 50.0 & 47.1 & 57.1 & \textbf{51.6} \\
%  & Status & 15 & 53.3 & 50.0 & 20.0 & 28.6 & 44.4 & 26.7 & 33.3 & 50.0 & 26.7 & 34.8 & 15.4 & 26.7 & 19.5 & 50.0 & 33.3 & 40.0 & 35.3 & 40.0 & 37.5 & 41.2 & 46.7 & \textbf{43.8} \\
 
%  & Experiencer & 15 & 66.7 & 16.7 & 6.7 & 9.5 & 33.3 & 20.0 & 25.0 & 25.0 & 13.3 & 17.4 & 15.4 & 26.7 & 19.5 & 40.0 & 26.7 & 32.0 & 37.5 & 40.0 & 38.7 & 41.2 & 46.7 & \textbf{43.8} \\ \hline %\cline{1-2}
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Substance use \\ - alcohol / \\ drug / tobacco\end{tabular}} & Trigger & 78 & 86.4 & 92.5 & 79.5 & \textbf{85.5} & 84.2 & 82.1 & 83.1 & 93.7 & 75.6 & 83.7 & 65.6 & 78.2 & 71.3 & 81.8 & 70.1 & 75.5 & 75.5 & 52.1 & 61.7 & 71.7 & 92.2 & 80.7 \\
%  & Status & 78 & 85.7 & 88.1 & 75.6 & 81.4 & 80.0 & 76.9 & 78.4 & 89.4 & 75.6 & \textbf{81.9} & 59.5 & 56.4 & 57.9 & 75.0 & 46.2 & 57.1 & 82.3 & 65.4 & 72.9 & 69.7 & 88.5 & 78.0 \\
%  & Experiencer & 78 & 73.2 & 80.6 & 69.2 & 74.5 & 81.6 & 79.5 & 80.5 & 87.9 & 74.4 & \textbf{80.6} & 59.2 & 37.2 & 45.7 & 75.0 & 46.2 & 57.1 & 81.8 & 69.2 & 75.0 & 71.4 & 89.7 & 79.5 \\ \hline %\cline{1-2}
% \multirow{3}{*}{Trauma} & Trigger & 33 & 88.9 & 72.0 & 54.5 & 62.1 & 52.8 & 57.6 & 55.1 & 84.2 & 48.5 & 61.5 & 52.9 & 54.5 & 53.7 & 100.0 & 42.4 & 59.6 & 50.0 & 3.6 & 6.7 & 83.3 & 60.6 & \textbf{70.2} \\
%  & Status & 33 & 88.9 & 60.0 & 45.5 & 51.7 & 52.8 & 57.6 & 55.1 & 61.5 & 48.5 & 54.2 & 46.7 & 42.4 & 44.4 & 50.0 & 3.0 & 5.7 & 100.0 & 42.4 & 59.6 & 75.0 & 54.5 & \textbf{63.2} \\
%  & Type & 33 & 84.6 & 64.0 & 48.5 & 55.2 & 50.0 & 54.5 & 52.2 & 61.5 & 48.5 & 54.2 & 50.0 & 39.4 & 44.1 & 50.0 & 3.0 & 5.7 & 100.0 & 39.4 & 56.5 & 79.2 & 57.6 & \textbf{66.7} \\ \hline % \cline{1-2}
 
% \multirow{3}{*}{\textbf{Overall}} & \textbf{--} & 1373 & 81.9 & 73.0 & 71.0 & 72.0 & 81.3 & 77.1 & 79.1 & 86.1 & 74.6 & \textbf{79.9} & 57.9 & 66.1 & 61.7 & 70.3 & 58.0 & 63.5 & 70.5 & 69.2 & 69.9 & 69.5 & 82.1 & 75.3 \\
%  & \textbf{Trigger} & 529 & 85.1 & 86.5 & 73.7 & 79.6 & 83.5 & 79.2 & 81.3 & 89.8 & 76.3 & \textbf{82.5} & 66.8 & 78.6 & 72.2 & 83.3 & 76.5 & 79.7 & 75.3 & 64.9 & 69.7 & 78.2 & 86.5 & 82.2 \\
%  & \textbf{Arguments} & 844 & 80.0 & 66.1 & 69.3 & 67.7 & 80.0 & 75.7 & 77.8 & 83.8 & 73.6 & \textbf{78.4} & 52.0 & 58.2 & 54.9 & 60.6 & 46.4 & 52.6 & 68.4 & 71.4 & 69.9 & 64.6 & 79.3 & 71.2 \\ \hline
 
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hallucination \\ rate\end{tabular}}} & \textbf{Tigger} & -- & -- & \multicolumn{3}{c|}{--} & \multicolumn{3}{c|}{3.9} & \multicolumn{3}{c|}{3.9} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{5.9} & \multicolumn{3}{c|}{5.4} & \multicolumn{3}{c}{4.1} \\
%  & \textbf{Arguments} & -- & -- & \multicolumn{3}{c|}{--} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{} & \multicolumn{3}{c}{} \\ \hline
% \end{tabular}

==> tables/performance_event_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[]
\small
\setlength{\tabcolsep}{2pt}
\resizebox{0.5\textwidth}{!}{% use resizebox with textwidth
\begin{tabular}{lcccccc}
\hline
\multirow{3}{*}{\textbf{Event}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# \\ gold\\ labels\end{tabular}}} & \multicolumn{5}{c}{\textbf{Event extraction performance (F1)}} \\ \cline{3-7} 
 &  & \multicolumn{3}{c}{\textbf{Fine-tuning}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}In-context\\ learning\end{tabular}}} \\ \cline{3-7} 
 &  & \textbf{mSpERT} & \textbf{\begin{tabular}[c]{@{}c@{}}T5-\\  Event\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}T5-\\  2sQA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}GPT-\\  Event\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}GPT+\\ 3-shot\end{tabular}} \\ \hline % \cline{1-7}
 
Adoption & 9 & \textbf{84.2} & 82.4 & \textbf{84.2} & 58.1 & 54.5 \\
Edu. Acc. & 74 & 78.0 & 79.1 & 84.1 & 71.6 & \textbf{84.5} \\
Employment & 117 & 71.4 & 73.5 & 74.3 & 60.8 & \textbf{79.7} \\
Food. insec. & 8 & \textbf{93.3} & 87.5 & \textbf{93.3} & 53.3 & 73.7 \\
Living arrg. & 195 & 72.8\textsuperscript{\textdagger} & 69.7\textsuperscript{\textdagger} & \textbf{74.9}\textsuperscript{\textdagger} & 19.8 & 12.6 \\
Mental health & 15 & 9.5 & 8.3 & 17.4 & 21.1 & \textbf{37.5} \\
Subst. use & 78 & 75.9 & 75.0 & \textbf{80.6}\textsuperscript{\textdagger} & 45.9 & 78.0 \\
Trauma & 33 & 51.7 & 51.5 & 53.3 & 55.2 & \textbf{59.6} \\ \hline
\begin{tabular}[c]{@{}l@{}}Micro\\ Avg\end{tabular} & 529 & 71.6\textsuperscript{\textdagger} & 70.4\textsuperscript{\textdagger} & \textbf{74.7}\textsuperscript{\textdagger} & 42.6 & 54.0\textsuperscript{\textdagger} \\ \hline
\end{tabular}


}
\caption{Model performance F1 (\%) with the \textit{event-level} evaluation on the PedSHAC withheld test set. The symbol \textsuperscript{\textdagger} marks with significantly higher performance than GPT-Event. The highest performance in each row is in boldface.}
\label{tab:eventF1}
\end{table}
